Managing Human Factors in Automated Vehicle Development: Towards Challenges and Practices

Due to the technical complexity and social impact, automated vehicle (AV) development challenges the current state of automotive engineering practice. Research shows that it is important to consider human factors (HF) knowledge when developing AVs to make them safe and accepted. This study explores the current practices and challenges of the automotive industries for incorporating HF requirements during agile AV development. We interviewed ten industry professionals from several Swedish automotive companies, including HF experts and AV engineers. Based on our qualitative analysis of the semi-structured interviews, a number of current approaches for communicating and incorporating HF knowledge into agile AV development and associated challenges are discussed. Our findings may help to focus future research on issues that are critical to effectively incorporate HF knowledge into agile AV development.

==> recomendations.tex <==





c) Test system with HF perspective: It was suggested
to improve the process to test the system regularly from
HF perspective, particularly in agile development. 


“Not sure we are good with agile yet, but ideally, we should
get even improvements through improved testing. As long as you
can include an HF expert, then all should be fine in the larger
picture.”


“A good start is to have a HF champion in each project. In
our project we do have a few test engineers. Perhaps there,
HF knowledge would benefit most. Defining those tests and
articulating what matters would be great to spread the knowledge.
It does not appear to be feasible to have one HF person per team,
but one HF expert per project (40 people) or office (100-200)
would be good.”


